VideoSketcher: Sequential Sketch Generation Using Video Model Priors

Sketching is inherently sequential: strokes are drawn progressively to explore and refine ideas. Yet most generative approaches treat sketches as static images, ignoring the temporal process underlying creative exploration. Modeling this sequential structure remains challenging: prior methods either rely on large-scale human-drawn datasets with limited diversity, or use large language models (LLMs) to produce drawing instructions, often at the cost of visual fidelity. We present VideoSketcher, a method for generating high-quality sketching processes by adapting pretrained text-to-video diffusion models to the sparse, continuous nature of sketch formation. Our key insight is that LLMs and video diffusion models offer complementary strengths: LLMs act as semantic planners that decompose concepts into step-by-step instructions, while video diffusion models serve as powerful "renderers" that translate them into temporally coherent sketch sequences. We introduce a two-stage fine-tuning strategy that decouples temporal structure from visual appearance: stroke ordering is learned from synthetic shape compositions, while style is distilled from as few as seven hand-drawn examples. Despite minimal supervision, our method can generate diverse, high-quality sequential sketches that faithfully follow specified drawing orders. Our framework naturally extends to brush style control and autoregressive generation, supporting artistic applications.

==> figs_tex/ablation_qualitative.tex <==
\begin{figure*}[t]
\centering
\setlength{\tabcolsep}{0.5pt}
\renewcommand{\arraystretch}{0.2}
\small

\begin{tabular}{r c c}

 & \parbox[c]{0.43\linewidth}{\centering \emph{Cat: 1. Body. 2. Head. 3. Ears. 4. Face details. 5. Legs. 6. Tail.}} 

 & \parbox[c]{0.43\linewidth}{\centering \emph{Cat: 1. Head. 2. Ears. 3. Body. 4. Legs. 5. Tail. 6. Face details.}}  \\[2pt]

\raisebox{0.3cm}{Primitives Only} &
\includegraphics[width=0.4\linewidth]{figs/ablations/12_shapes_cat.png} &
\includegraphics[width=0.4\linewidth]{figs/ablations/11_shapes_cat.png} \\

\raisebox{0.3cm}{7 Human Sketches Only} &
\includegraphics[width=0.4\linewidth]{figs/ablations/12_cat_7sketches.png} &
\includegraphics[width=0.4\linewidth]{figs/ablations/11_cat_7sketches.png} \\

\raisebox{0.3cm}{Full} &
\includegraphics[width=0.4\linewidth]{figs/ablations/12_cat_FT.png} &
\includegraphics[width=0.4\linewidth]{figs/ablations/11_cat_FT.png}

\end{tabular}
\vspace{-10pt}
\caption{\textbf{Ablation study qualitative comparison.} We compare sketching processes from models trained only on geometric primitives, only on real sketches, and the full two-stage model. The full model combines the strengths of both baselines, producing visually appealing sketches that follow the specified order.}
\label{fig:ablation_comaprison}
\vspace{-10pt}
\end{figure*}


==> figs_tex/autoregressive_comp.tex <==
\begin{figure}[t]
\centering
\setlength{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{0.9}
\small

\newcommand{\trimimg}[1]{%
  \frame{\includegraphics[width=0.18\linewidth, trim=3.5cm 0pt 3.5cm 0pt, clip]{#1}}%
}
\includegraphics[width=0.75\linewidth]{figs/autoregressive/co-drawing/demo_screenshot.png}\\[6pt]

\begin{tabular}{ccccc}

\multicolumn{1}{c}{User} &
\multicolumn{1}{c}{Model} &
\multicolumn{1}{c}{User} &
\multicolumn{1}{c}{Model} &
\multicolumn{1}{c}{User} \\

\trimimg{figs/autoregressive/co-drawing/a0000_sketch_last.png} &
\trimimg{figs/autoregressive/co-drawing/a0001_model_last.png} &
\trimimg{figs/autoregressive/co-drawing/a0002_sketch_last.png} &
\trimimg{figs/autoregressive/co-drawing/a0003_model_last.png} &
\trimimg{figs/autoregressive/co-drawing/a0004_sketch_last.png} \\


\multicolumn{1}{c}{Model} &
\multicolumn{1}{c}{User} &
\multicolumn{1}{c}{Model} &
\multicolumn{1}{c}{User} & 
\multicolumn{1}{c}{Model}\\

\trimimg{figs/autoregressive/co-drawing/b0000_model_last.png} &
\trimimg{figs/autoregressive/co-drawing/b0001_sketch_last.png} &
\trimimg{figs/autoregressive/co-drawing/b0002_model_last.png} &
\trimimg{figs/autoregressive/co-drawing/b0003_sketch_last.png} &
\trimimg{figs/autoregressive/co-drawing/b0004_model_last.png} \\

\end{tabular}

\vspace{-9pt}
\caption{\textbf{Co-Drawing.}  Top: our interactive demo, where users draw alongside the model in real time. Bottom: turn-based co-drawing for ``a creature.''}
\vspace{-0.4cm}
\label{fig:ar_comparison}
\end{figure}


==> figs_tex/brush_control.tex <==
\begin{figure}[t]
\centering
\setlength{\tabcolsep}{0pt}
\renewcommand{\arraystretch}{0.6}
\small
\begin{tabular}{c}
    \includegraphics[width=0.875\linewidth]{figs/brushes_icecream.pdf} \\
\end{tabular}
\vspace{-9pt}
\caption{\textbf{Brush style control via visual prompting.} Left: brushes and colors seen during training. Right: generalization to unseen brushes and colors.
}
\vspace{-0.275cm}
\label{fig:brush_control}
\end{figure}


==> figs_tex/clip_recognition_over_time.tex <==
\begin{figure}
    \centering
    \includegraphics[
        width=0.9\linewidth,
        trim=0pt 0pt 0pt 0.8cm,
        clip
    ]{figs/clip_score_plot.pdf} \\[-0.45cm]
    \caption{\textbf{CLIP-based recognition over the sketching process.} Our method gradually increases semantic recognizability as the sketch progresses, in contrast to baselines that either collapse temporal progression or attain lower recognition. Shaded areas indicate variance across samples.}
    \label{fig:clip_score_plot}
    \vspace{-0.25cm}
\end{figure}


==> figs_tex/limitations.tex <==
\begin{figure}[t]
\centering
\footnotesize

\begin{subfigure}[t]{\linewidth}
    \centering
    \caption{Multiple strokes per frame}
    \includegraphics[width=0.875\linewidth]{figs/limitations/limitation_multi_stroke.png}
\end{subfigure}

\vspace{-4pt}

\begin{subfigure}[t]{0.295\linewidth}
    \centering
    \caption{Prompt adherence}
    \includegraphics[width=\linewidth]{figs/limitations/limitation_tiger.png}
    \emph{``A tiger roaring''}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.295\linewidth}
    \centering
    \caption{Limited knowledge}
    \includegraphics[width=\linewidth]{figs/limitations/limitation_function.png}
    \emph{``$y=x^2$''}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.295\linewidth}
    \centering
    \caption{AR quality gap}
    \includegraphics[width=\linewidth]{figs/limitations/limitation_ar.png}
    \emph{``A lobster''}
\end{subfigure}
\vspace{-10pt}
\caption{\textbf{Limitations.} (a) Multiple strokes may appear together (in red). (b) Model's prior can override prompt. (c) Concepts outside the video model's knowledge are incorrectly depicted. (d) Reduced quality for AR outputs.}
\label{fig:limitations}
\vspace{-12pt}
\end{figure}


==> figs_tex/our_results.tex <==
\begin{figure*}[t]
\centering
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.2}
\small


\begin{tabular}{c c}
  \lefttxt{``An Amsterdam\\ canal.''} &
  \includegraphics[width=0.85\linewidth]{figs/our_results/amsterdam_canal_following_Ours-FT-1_0.png} \\[2pt]

  \lefttxt{``A Rome street\\ with a cat.''} &
  \includegraphics[width=0.85\linewidth]{figs/our_results/rome_street_cat_Ours-FT-2_0.png} \\[2pt]

  \lefttxt{``A Tokyo alley\\ with lanterns.''} &
  \includegraphics[width=0.85\linewidth]{figs/our_results/tokyo_alley_lanterns_Ours-FT-2_1.png}
\end{tabular}

\vspace{-7pt}
\caption{\textbf{Qualitative results.} Results generated with our fine-tuned video model. Full video results are provided in the supplementary materials.}
\label{fig:our_results}
\vspace{-4pt}
\end{figure*}


==> figs_tex/qualitative_comparisons.tex <==
\begin{figure}
\centering
\setlength{\tabcolsep}{2pt} %
\renewcommand{\arraystretch}{0.2} %
\small

\newcommand{\rowlab}[1]{\rotatebox{0}{\strut #1}}

\begin{tabular}{r c c c}

\raisebox{0.175cm}{\rotatebox{90}{\begin{tabular}{c} Naive\\Wan2.1 \end{tabular}}} &
\includegraphics[width=0.85\linewidth]{figs/comparisons/giraffe/Wan2.1-T2V-14B.png} \\

\raisebox{0.175cm}{\rotatebox{90}{\begin{tabular}{c} Paints\\Undo \end{tabular}}} &
\includegraphics[width=0.85\linewidth]{figs/comparisons/giraffe/PaintsUndo.png} \\

\raisebox{0.175cm}{\rotatebox{90}{\begin{tabular}{c} Sketch\\Agent \end{tabular}}} &
\includegraphics[width=0.85\linewidth]{figs/comparisons/giraffe/SketchAgent.png} \\

\raisebox{0.0cm}{\rotatebox{90}{\begin{tabular}{c} Human\\(QuickDraw) \end{tabular}}} &
\includegraphics[width=0.85\linewidth]{figs/comparisons/giraffe/QuickDraw.png} \\

\raisebox{0.3cm}{\rotatebox{90}{{\textbf{Ours}}}} &
\includegraphics[width=0.85\linewidth]{figs/comparisons/giraffe/Ours-FT.png} \\ 


\end{tabular}
\vspace{-9pt}
\caption{\textbf{Qualitative comparison} of sketch generation across methods. The concept depicted is ``a giraffe''.
}
\label{fig:qual_comparison}
\vspace{-10pt}
\end{figure}


==> sec/1_intro_b.tex <==
\section{Introduction}\label{sec:introduction}
Sketches and drawings are a fundamental medium for exploring, communicating, and refining ideas~\cite{fan2023drawing,tversky2013visualizing}. Their expressive power lies not only in the final result, but also in the \emph{process} of drawing itself: through the gradual accumulation of strokes, creators externalize thoughts, explore alternatives, and iteratively refine emerging concepts~\cite{goldschmidt1992serial,tversky2003sketches}. Computational models that generate sketches as sequential processes, rather than as static images, therefore have the potential to enable richer forms of human-machine interaction, including visual brainstorming, real-time feedback, and collaborative prototyping through a natural visual medium.

Yet modeling the \emph{process} of drawing --- rather than only its static final output --- remains a significant challenge. The goal is not simply to generate strokes gradually, but to do so in a \emph{meaningful, human-like order}, where structure is built through semantically coherent progressions rather than arbitrary stroke sequences.
Prior approaches have taken important steps toward this goal, but face fundamental limitations. SketchRNN~\cite{SketchRNN} introduced autoregressive sketch generation trained directly on human drawing sequences, enabling the model to learn stroke ordering from data. However, this approach relies on millions of human-drawn sketch sequences and is restricted to a fixed set of object categories with limited stylistic diversity.

More recently, SketchAgent~\cite{SketchAgent_Vinker2025} demonstrated that multimodal large language models (LLMs) possess a surprising capacity for sequential sketch generation without requiring sketch-specific training. By prompting an LLM to output stroke coordinates as textual commands, SketchAgent generates drawings across a broad range of concepts, leveraging the model’s semantic understanding to produce meaningful stroke orderings. However, this approach has an inherent bottleneck: while LLMs excel at deciding \emph{what} to draw and in what \emph{order}, they struggle with \emph{how} to draw it. As a result, the generated sketches, although semantically coherent, tend to be overly simplistic and often lack visual quality.

In this work, we leverage text-to-video diffusion models for sequential sketch generation. Trained on large-scale video data, these models encode rich priors over visual appearance, motion, and temporal coherence. Our key insight is that video diffusion models and large language models offer \emph{complementary} strengths for this task: LLMs provide semantic understanding that enables meaningful planning and stroke ordering, but are limited as visual renderers, whereas video diffusion models excel at high-quality visual synthesis but lack an intrinsic notion of drawing order. We combine these capabilities by using a video diffusion model as the ``renderer'', guided by an LLM that specifies what to draw and in which order.

We represent a sketch sequence as a short video in pixel space, in which black strokes are progressively drawn on a blank canvas. Despite the apparent gap between photorealistic video content and abstract hand-drawn sketches, we show that video diffusion models can be effectively distilled into sketch-like behavior using only a \emph{handful} of carefully constructed examples.

A key challenge in this distillation process is teaching the model not only what sketches should look like, but also how they should unfold over time, following the ordering instructions specified by an LLM. Direct fine-tuning on hand-drawn sketches alone does not reliably yield such temporal control. To address this, we introduce a two-stage fine-tuning strategy.
In the first stage, we train the model on a small, manually constructed dataset of basic geometric primitives, such as ovals, rectangles, triangles, and curves, arranged to exhibit fundamental compositional relationships inspired by Gestalt principles~\cite{koffka2013principles}, including containment, adjacency, overlap, and grouping. Each composition is rendered using multiple drawing orders, teaching the model both a ``visual vocabulary'' of primitives and the ability to follow text-specified stroke sequences.
In the second stage, we adapt the model to the visual style of hand-drawn sketches using as few as seven examples, transferring the learned temporal control to the target sketch domain.

Despite the extremely limited amount of real sketch data, our method generates high-quality sequential sketches across a diverse range of concepts, accurately following the ordering specified by the text prompt while exhibiting substantially richer visual detail and stronger temporal coherence (see~\Cref{fig:teaser}).

Beyond diffusion-based generation, we show that our distilled model can bootstrap autoregressive sketch generation by synthesizing additional training data, enabling interactive scenarios such as collaborative co-drawing. We also demonstrate that video diffusion models support brush style conditioning, allowing users to control stroke appearance using a simple visual cue. This enables brush-level control within a pixel-based generation framework --- a capability usually associated with parametric stroke representations --- and further illustrates the flexibility of video diffusion models for modeling drawing processes.

Together, these results suggest that pretrained video diffusion models offer a powerful and flexible prior for modeling drawing processes, providing a new perspective on sequential sketch generation that does not rely on large-scale sketch datasets or explicit parametric stroke representations.


==> sec/2_prev_work.tex <==
\section{Related Work}\label{sec:prev_work}

\paragraph{Sequential sketch generation.}
A common approach to sequential sketch generation represents sketches as explicit stroke sequences and trains models on large collections of human drawing data~\cite{SketchRNN, SketchGPT, VQ-SGen, DiffSketcher, StrokeFusion}.
Among these, SketchRNN~\cite{SketchRNN} pioneered this direction by introducing the QuickDraw dataset~\cite{quickDrawData}, the largest collection of human-drawn sequential sketches. 
However, approaches that learn directly from such datasets are inherently constrained by the predefined categories and styles present in the training data. For QuickDraw, for example, this corresponds to at most 340 object categories with predominantly non-professional drawing quality.

To overcome this bottleneck, recent work has explored the use of large language models (LLMs)~\cite{minaee2025largelanguagemodelssurvey,zhao2025surveylargelanguagemodels} to guide sequential visual generation.
Because these models operate primarily over text, they are typically paired with external systems that translate language outputs into drawing actions or canvas edits~\cite{hu2024visual,shaham2024multimodal,yang2023idea2img,wu2023visual,svg_spec}. 
SketchAgent~\cite{SketchAgent_Vinker2025} frames sketch generation as a language-driven process, in which a multimodal LLM produces drawing instructions that are executed on a canvas. While this enables flexible, text-conditioned sequential sketching beyond fixed object categories, sketch quality remains constrained by a textual bottleneck: although LLMs excel at semantic reasoning and planning, they lack strong spatial and visual priors. As a result, the generated sketches tend to be overly simple and exhibit a child-like drawing style. In contrast, our method addresses this limitation by leveraging the rich visual priors of video models as powerful renderers of LLM commands, enabling substantially richer visual detail while preserving text-specified stroke ordering.

Recently, video models have been applied to painting reconstruction. \emph{PaintsUndo}~\cite{paintsundo} and \emph{PaintsAlter}~\cite{paintsalter} aim to recover or reverse the creation process of an existing painting by predicting intermediate states conditioned on a completed image. While effective for painting reconstruction, these methods rely on $~20k$ Procreate recordings for training and produce relatively coarse, frame-level progressions. 
In contrast, we pursue a fundamentally different goal: generating new sketches from text with explicit, stroke-by-stroke progression. This enables open-ended creative exploration in which the final result emerges through the drawing process rather than being predetermined. The slower, stroke-level progression naturally supports co-creation, allowing users to interpret and contribute as the sketch unfolds. Crucially, we demonstrate that this can be achieved using only a handful of training examples.

Finally, a related line of work uses reinforcement learning to train painting agents that produce sequential paintings for various tasks~\cite{ganin2018synthesizing,mellor2019unsupervised,mihai2021learning,zhou2018learning}. However, these methods are not designed to model semantically meaningful stroke ordering and are typically restricted to narrow domains, such as faces or a small set of predefined objects.


\vspace{-0.05cm}
\paragraph{VLM-guided vector sketch synthesis}
Large pretrained diffusion and vision-language models (VLMs) provide strong semantic priors and have been widely used for static sketch and vector graphic generation~\cite{Radfordclip,rombach2022highresolution,sdxl2023,saharia2022photorealistic,schuhmann2022laion5b}.
A prominent line of work formulates sketch synthesis as an optimization problem over parametric vector strokes, which are iteratively refined under pixel-space guidance from pretrained models, typically large-scale VLMs, using differentiable rasterization~\cite{vinker2022clipasso,jain2023vectorfusion,NEURIPS2023_DiffSketcher,svgdreamer_xing_2023,Text-to-Vector2024Zhang,Vinker_2023_ICCV,3Doodle2024Choi,gal2023breathing,arar2025swiftsketch,diffvg}.

While effective at producing semantically aligned static sketches, these approaches optimize all strokes jointly toward a final objective and do not explicitly model the temporal drawing process. As a result, they lack meaningful stroke ordering and are less suitable for interactive sketching scenarios.


\vspace{-0.05cm}
\paragraph{Video priors and interactive video generation}
Recent advances in video generation show that models trained on large-scale video data capture strong temporal structure and can serve as effective priors for new visual tasks~\cite{Wan2.1,HunyuanVideo,LTX-Video,openai2025sora2,veo3technicalreport,video-zero-shot-reasoners}. We build on this insight by adapting pretrained video generation models to learn sketching behavior in a few-shot setting.

Standard video diffusion models generate entire video clips jointly, making inference computationally expensive and limiting interactivity. Recent work, therefore, explores causal or autoregressive video models that use temporally causal attention to generate frames sequentially~\cite{Causvid,SelfForcing,LongLive,chen2024diffusion,yin2024improved,yin2024one,cui2025self,yin2025slow}. While these models may trade some visual fidelity for efficiency, they are better suited for human-in-the-loop applications. We adopt such an autoregressive model for sequential sketch generation, enabling collaborative sketching.


==> sec/3_method_new.tex <==
\setlength{\abovedisplayskip}{4pt}
\setlength{\belowdisplayskip}{4pt}
\setlength{\abovedisplayshortskip}{2pt}
\setlength{\belowdisplayshortskip}{2pt}

\section{Method}\label{sec:method}


 



Our goal is to generate a video depicting a sequential sketching process conditioned on a text prompt, in which strokes follow the specified ordering and exhibit natural drawing behavior. We build on the strong priors of a pretrained text-to-video diffusion model~\cite{Wan2.1} and adapt them to the sketch domain through a two-stage fine-tuning strategy. As we show, careful data construction is central to effective distillation: by disentangling stroke ordering from visual appearance across stages, the model learns complex sketching behavior from only a handful of examples.

\subsection{Sketch Representation and Construction}
We represent a sketch sequence as a short video $V \in \mathbb{R}^{K \times H \times W \times 3}$ in pixel space, depicting black strokes progressively drawn on a blank canvas. A natural sketching appearance requires modeling not only the global ordering of strokes, but also the local, continuous drawing within each stroke, mimicking the motion of a human hand across the canvas.
To achieve this, we construct training data by capturing sketching processes as SVGs (Scalable Vector Graphics)~\cite{cai2023delving} and rendering them via procedural stroke animation. An artist draws each sketch in Adobe Illustrator, which records both the stroke sequence and the drawing trajectory of each individual path. We then parse these SVG files and render them as videos by animating each stroke to appear gradually along its path, producing temporally structured sketching videos that preserve both stroke ordering and within-stroke progression (see~\Cref{fig:svg_parsing}).

This representation offers several advantages. First, it enables fine-grained temporal control by ensuring that at most one stroke is introduced per frame, avoiding artifacts such as simultaneous stroke appearance. Second, it naturally accommodates different video model requirements, including resolution, frame count, and random seed, through simple adjustments to the rendering parameters. Third, as shown in~\Cref{sec:brush_control}, the parametric nature of SVGs enables the same stroke sequence to be rendered with different brush styles, providing additional training data for brush conditioning with no further manual effort.

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{figs/svg-to-vid.pdf} \\[-0.25cm]
    \caption{\textbf{SVG-to-video sketch representation.} SVG paths are parsed and rendered sequentially into a video in which strokes are progressively drawn on a canvas. Each frame introduces at most one new stroke, ensuring clean temporal structure while enabling pixel-based video diffusion modeling.}
    \label{fig:svg_parsing}
    \vspace{-0.35cm}
\end{figure}

Although SVGs offer a compact and structured representation, directly generating parametric sketches typically requires specialized architectures or inference-time optimization, often relying on large datasets and without explicitly modeling stroke order. By operating in pixel space, we instead leverage the full generative capacity of pretrained video diffusion models while still producing clean, parametric-like visual quality through sequential generation.


\subsection{Text Prompt Construction}
The text prompt must specify not only what to draw, but also the order in which elements should be drawn. We adopt a prompt format consisting of a brief description of the subject followed by an explicit, numbered sequence of drawing steps. For example:

\begin{adjustwidth}{1em}{1em}
\footnotesize
\textit{
\\[0.01cm]
Step-by-step sketch process of a desk lamp, following this drawing order:\\
1. Lampshade – a cone-shaped top part that directs the light downward.\\
2. Light bulb - \dots\\
\dots\\
7. Light beam emanating from the bulb.
}\\
\end{adjustwidth}

Each step describes a semantic component of the object rather than low-level geometric primitives, and the ordering reflects natural drawing logic, such as sketching main forms before details and structural elements before secondary details.

At inference time, we use an LLM~\cite{OpenAI2026GPT5} to generate structured drawing plans from high-level user input. This design exploits the LLM’s strengths in semantic decomposition and planning~\cite{SketchAgent_Vinker2025}, while delegating visual realization and temporal rendering to the video diffusion model.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/temp_pipe_2.pdf} \\[-0.15cm]
    \caption{\textbf{Two-stage fine-tuning scheme.} Left: synthetic sketches composed of simple geometric primitives teach drawing ``grammar'' and stroke ordering, independently of appearance. Right: a small set of human-drawn sketches of real-world objects adapts the model to a target visual style.}
    \vspace{-0.3cm}
    \label{fig:shapes}
\end{figure}

\subsection{Two-Stage Finetuning}
While video diffusion models encode strong visual priors, they lack an intrinsic notion of meaningful drawing order. As we demonstrate, naive fine-tuning on sketch videos can produce sketch-like appearance but often yields arbitrary or inconsistent stroke sequences. The central challenge, therefore, is to achieve both high visual fidelity and explicit temporal control over the sketching process.

We address this with a two-stage fine-tuning strategy that disentangles these objectives. Before training on real-world sketches, we first teach the model a basic drawing ``grammar'': simple shapes, their spatial relationships, and how to follow ordering instructions. This design is inspired by how people learn to draw, starting with simple shapes and compositional rules before progressing to more complex subjects~\cite{kellog1969analyzing,edwards1989drawing}.

In both stages, fine-tuning uses standard video diffusion training with rectified flow matching. We do not modify the diffusion architecture or introduce task-specific losses; instead, learning is driven entirely by carefully constructed data, allowing the pretrained model to acquire sketch-specific behavior through data alone.


\input{figs_tex/our_results}


\paragraph{Learning the ``Grammar'' of Shape Compositions}
We construct a small dataset of simple geometric primitives, including circles, ellipses, triangles, rectangles, polygons, curves, and lines, encoded as SVGs and rendered into sketch videos following the representation described in the previous section. These primitives are arranged in diverse spatial configurations inspired by Gestalt principles, such as containment (a circle inside a rectangle), adjacency (shapes placed side by side), overlap (partially occluding forms), and grouping (clustered elements). These relationships reflect the compositional building blocks underlying more complex sketches (see~\Cref{fig:shapes}). For each configuration, we vary the order in which the shapes are drawn, producing three distinct temporal variations per sketch.

Because the shapes are visually simple and semantically neutral, this dataset minimizes appearance-related variability and encourages the model to focus on learning temporal stroke ordering rather than object-specific visual details. Text prompts explicitly describe the intended drawing order, enabling the model to learn a direct correspondence between linguistic ordering cues, such as ``first draw \dots, then draw \dots,'' and the temporal sequence of stroke additions. 
This synthetic pretraining stage is critical: as we demonstrate in~\Cref{sec:ablation}, incorporating this initial fine-tuning stage with synthetic shape compositions significantly improves ordering fidelity.

\paragraph{Distilling Sketch Appearance}
While training on primitive shape compositions is effective for learning stroke ordering, models trained only on such data tend to compose drawings directly from these primitives, resulting in sketches that lack the desired visual appearance. To bridge this gap, we perform a second fine-tuning stage using a small set of seven real-world sketches drawn by an artist: a lamp, car, chair, tree, cup, butterfly, and flower (see~\Cref{fig:shapes}).

This stage adapts the model to the target visual aesthetic and level of abstraction that we aim to produce at inference time. Because the model has already learned to follow explicit ordering instructions during the synthetic pretraining stage, this fine-tuning primarily transfers appearance information rather than requiring the model to infer stroke ordering from a limited number of examples.



\subsection{Brush Conditioning}
We further demonstrate the flexibility of video models as priors for sequential sketch generation through a brush conditioning application. The goal is to allow users to control sketch style—both brush type and color—via a simple visual cue. Specifically, we provide the model with a small brush exemplar placed in the top-left corner of the canvas (see~\Cref{fig:teaser}), which guides stroke appearance throughout the sketching process without requiring an explicit parametric brush representation.

Training data is constructed using the same SVG sketches described earlier, rendering each sketch with multiple brush styles and colors, using six distinct brushes and eight colors in total. We then fine-tune an image-to-video diffusion model \cite{Wan2.1} using the same training procedure, with the first frame provided as a conditioning input image. In all cases, the first frame consists of a blank canvas augmented with the brush sample in the top-left corner, allowing the model to infer the desired brush appearance directly from the visual prompt.


\subsection{Autoregressive Modeling}
Our primary approach relies on diffusion-based video models that generate the entire sketch sequence jointly rather than predicting frames sequentially. In contrast, an autoregressive formulation --- where each frame is conditioned on previously generated frames --- is particularly well-suited for interactive sketching. Because sketching is inherently sequential, with each stroke building on the current canvas, this paradigm naturally aligns with drawing-based, user-in-the-loop interaction.

While autoregressive video models are less mature than diffusion-based approaches, recent work has demonstrated promising progress \cite{Causvid,SelfForcing,chen2024diffusion,yin2024improved,yin2024one,cui2025self}. As these models continue to improve, our framework remains directly applicable, which we demonstrate by adapting our approach to an autoregressive video model.

A key challenge in autoregressive modeling is the need for substantially larger, high-quality training datasets~\cite{Causvid}. To address this, we use our diffusion-based sketch model, trained on a small set of real-world sketches, to generate a larger synthetic sketch dataset. This synthetic data is then used to fine-tune an autoregressive model, enabling sequential sketch generation in the autoregressive setting.






==> sec/5_results_v2.tex <==
\input{tables/textcond}

\section{Results}
Our method generates diverse sequential sketches, ranging from single objects to complex multi-element scenes, as shown in~\Cref{fig:teaser,fig:our_results,fig:additional_our_results}. Despite being trained on only 7 real sketches, it generalizes to complex scenes, including streets, canals, and alleys with multiple buildings, characters, and vehicles, producing clean lines, coherent perspective, and semantically meaningful stroke ordering (e.g., large structures first, fine details last). Moreover, as shown in~\Cref{fig:additional_results_diversity}, our approach supports diverse outputs, either by varying the initial noise for a fixed prompt or by modifying the specified action.

\subsection{Text-Conditioned Sketch Generation}\label{sec:text_generation}
We quantitatively evaluate how well the generated sketches depict the intended category. Following the evaluation protocol of SketchAgent~\shortcite{SketchAgent_Vinker2025}, we randomly sample $50$ categories from the QuickDraw dataset~\cite{quickDrawData}, and generate two sketches per category using different random seeds, yielding 100 sketches in total. 
We compare our method against several baselines, including naive prompting of Wan2.1~\cite{Wan2.1}, PaintsUndo~\cite{paintsundo}, SketchAgent~\cite{SketchAgent_Vinker2025}, and human-drawn sketches from the QuickDraw dataset. Since PaintsUndo requires a final frame as input, we provide final frames generated by FLUX2~\cite{flux-2-2025}.


\input{figs_tex/qualitative_comparisons}

To quantify how well generated sketches depict the intended category, we follow standard practice~\shortcite{vinker2022clipasso,Vinker_2023_ICCV,SketchAgent_Vinker2025} and employ a CLIP ViT-B/32 zero-shot classifier on the final frame of each sequence. We report average Top-1 and Top-5 classification accuracy in~\Cref{tab:CLIPscore}.
Our method achieves 82\% Top-1 accuracy, substantially outperforming SketchAgent (48\%) and human QuickDraw sketches (52\%), while reaching 96\% Top-5 accuracy compared to 71\% and 70\%, respectively. These results indicate that the fine-tuned video model generalizes effectively to a wide range of categories far beyond the seven sketches used during training.

We note that PaintsUndo attains high recognition scores because it is conditioned on a final image and reconstructs intermediate states that closely resemble the target, rather than generating sketches from text alone. As such, its performance is not directly comparable to methods that synthesize sketches from scratch. Wan 2.1 also achieves high final-frame recognition but, as shown in~\Cref{sec:sequential}, fails to produce meaningful stroke-by-stroke progression, yielding nearly identical frames throughout the sequence. In contrast, our method produces both recognizable final sketches and coherent drawing processes, as shown in~\Cref{fig:qual_comparison,fig:additional_qual_comparison}. 

\subsection{Sequential Sketching}\label{sec:sequential}
Beyond semantic alignment with the text prompt, we evaluate the quality of the sketching process itself. As shown in~\Cref{fig:ordering_diversity}, our method produces clean, stroke-by-stroke progressions in which strokes are added incrementally according to the specified order. Varying the text instructions for the same concept results in distinct sketching trajectories, demonstrating control over stroke ordering.

To assess whether the temporal progression is semantically meaningful, we measure CLIP-based category recognition as a function of video progress, as shown in~\Cref{fig:clip_score_plot}. Representative frames are visualized in~\Cref{fig:qual_comparison,fig:additional_qual_comparison} and in the supplementary material.

\input{figs_tex/clip_recognition_over_time}


A naive prompting of Wan2.1 (gray) produces near-identical frames throughout the sequence, resulting in a flat recognition curve. PaintsUndo (green) saturates rapidly, reaching high recognition early in the video, which reflects its undo-based formulation where detailed structure appears upfront. While effective for its intended task. In addition, PaintsUndo produces detailed, painting-like outputs rather than the clean, vector-like sketches we target.
SketchAgent (red) more closely follows human-like progression, but its outputs are often overly simplistic and sometimes fail to convey recognizable concepts (e.g., the cow example in~\Cref{fig:additional_qual_comparison}).

Our method closely tracks human progression while achieving substantially higher final accuracy (82\% vs. 52\% Top-1). As shown in~\Cref{fig:qual_comparison}, sketches evolve through semantically meaningful stages that follow human-like ordering, such as drawing the body before the neck and head, while producing more detailed final appearances.

\input{figs_tex/brush_control}


\subsection{Brush Style Control}\label{sec:brush_control}
Beyond stroke ordering, our video-based formulation offers flexibility in visual style.
As shown in~\Cref{fig:brush_control,fig:additional_brush}, conditioning on a brush exemplar in the first frame allows the model to reproduce the target brush's color and texture throughout the sketch. Notably, this generalizes to brush styles and colors not seen during training. 

To quantitatively evaluate generalization to unseen brush styles, we apply five unseen colors and five unseen brushes to sketches from 30 object categories, using two random seeds per category, for a total of 1,500 samples. To measure alignment between the user-provided brush exemplar and the generated strokes, following prior style transfer work~\cite{alaluf2024cross,deng2024zstarzeroshotstyletransfer,gatys2015neural}, we compute the average $\ell_2$ distance between Gram matrices extracted from three VGG-19 feature maps over stroke regions. As a baseline, we compare each output against all 25 brush exemplars used during evaluation, approximating the expected similarity to a randomly chosen brush.
Our method achieves an average distance of 3.73 compared to 7.29 for the random baseline (a 49\% reduction), indicating strong alignment with the target brush style.

\input{figs_tex/autoregressive_comp}

\input{figs_tex/ablation_qualitative}

\subsection{Autoregressive Generation}
Finally, we examine adapting our framework to autoregressive sketch generation, enabling interactive drawing scenarios that are difficult to support with diffusion-based models. As shown in~\Cref{fig:additional_results_ar}, the autoregressive model produces visually coherent sketches with clear stroke-by-stroke progression, although with slightly reduced visual fidelity compared to the diffusion-based approach.

We evaluate the autoregressive model using the same protocols as in \Cref{sec:text_generation,sec:sequential}. For final-frame recognition (\Cref{tab:CLIPscore}), it achieves 45\% Top-1 and 70\% Top-5 accuracy, comparable to human drawings (52\%/70\%) and SketchAgent (48\%/71\%). As shown in~\Cref{fig:clip_score_plot}, the recognition trajectory over time (purple) follows a gradual progression similar to human drawings (blue), indicating that the autoregressive formulation preserves meaningful temporal structure while enabling real-time interaction.

To demonstrate interactivity, we built a prototype collaborative sketching interface in which the user and the model alternate adding strokes to a shared canvas. As shown in~\Cref{fig:ar_comparison}, users can co-draw with the model in real time, with each adapting to the other’s contributions to produce coherent sketches. This result demonstrates the feasibility of turn-based co-drawing and highlights the potential of autoregressive video models for interactive sketch generation.


\subsection{Ablation Study}\label{sec:ablation}
We ablate a key design choice in our training procedure, namely, separating the learning of stroke ordering from sketch appearance. We compare three variants: our full two-stage model, a model trained only on synthetic geometric primitives, and a model trained only on seven human-drawn sketches.

Qualitative results (\Cref{fig:ablation_comaprison}) show that the two-stage model is necessary to achieve both reliable ordering control and realistic sketch appearance. Training only on primitives yields more consistent ordering but produces primitive-like, less aesthetic, recognizable drawings. In contrast, training only on real sketches improves visual style, but often fails to follow the specified ordering. Combining both stages yields the best performance, transferring ordering fidelity learned from synthetic compositions into the target domain.

\input{tables/ablation_clip}

To evaluate quantitatively, we measure CLIP Top-1 accuracy and ordering fidelity (\Cref{tb:ablation_joined}). Ordering fidelity is assessed via LLM-based head-to-head comparisons against the target ordering, with details provided in the supplementary materials. 



Quantitatively, the fully fine-tuned model achieves CLIP recognizability comparable to the model trained only on seven real sketches, indicating that visual aesthetic can be learned in a few-shot setting. The primitives-only model outperforms the real-sketch-only model in ordering fidelity, as expected given its focus on drawing grammar. When compared against both baselines, the fully fine-tuned model is strongly preferred in ordering fidelity, demonstrating that the two-stage training successfully combines ordering control with realistic sketch appearance. Although the full model outperforms the primitives-only model in ordering fidelity, this can be partly attributed to the simplicity of primitive-only sketches, which may not be recognizable enough for the LLM to reliably infer the drawn components and their order.




==> sec/6_conclusions.tex <==
\section{Limitations}
While our method supports flexible sequential sketch generation across a wide range of prompts and styles, it has several limitations (see ~\Cref{fig:limitations}).
Operating in pixel space provides less explicit structural control than parametric stroke representations, which can occasionally lead to violations of sketching constraints, such as multiple strokes appearing within a single frame. 
Second, prompt adherence is not guaranteed. When the model has a strong visual prior, it may deviate from the instructions. For example, in the ``tiger roaring'' prompt, the model changes the action late in the video and introduces color.
Performance also depends on the underlying video model’s concept knowledge, which is more limited than that of LLMs for specialized domains such as mathematics. 
Finally, while we demonstrate autoregressive sketch generation, the resulting outputs do not yet match the visual quality of the diffusion-based model, reflecting the present maturity of autoregressive video models.

\input{figs_tex/limitations}

\section{Conclusions}
We presented a data-efficient approach for sequential sketch generation that leverages pretrained text-to-video diffusion models as visual and temporal priors, guided by a large language model for semantic planning and stroke ordering.
By representing sketches as videos and decoupling stroke ordering from sketch appearance, our method generates coherent, text-conditioned drawing processes with meaningful temporal structure, even when trained on only a handful of examples. We further show that these video priors support extensions such as brush style conditioning and autoregressive sketch generation, enabling greater controllability and interactive applications. Together, these results highlight the potential of pretrained video diffusion models as general-purpose priors for modeling structured, temporally grounded creative processes.


==> tables/textcond.tex <==
\begin{table}[t]
\caption{\textbf{CLIP-based sketch recognition.} Average Top-1 and Top-5 accuracy of a CLIP zero-shot classifier evaluated on the last frame of 100 sketches from 50 categories. Results are reported as mean ± std across categories.\\[-0.7cm]}
\centering
\setlength{\tabcolsep}{6pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcc}
\toprule
Method & Top-1 & Top-5 \\
\midrule
Naive Prompting (Wan 2.1) 
& 0.92 $\pm$ 0.03 & 0.99 $\pm$ 0.01 \\

PaintsUndo (FLUX 2)~\cite{paintsundo} 
& 1.00 $\pm$ 0.00 & 1.00 $\pm$ 0.00 \\

SketchAgent~\cite{SketchAgent_Vinker2025} 
& 0.48 $\pm$ 0.05 & 0.71 $\pm$ 0.05 \\

Human (QuickDraw~\cite{quickDrawData}) 
& 0.52 $\pm$ 0.05 & 0.70 $\pm$ 0.05 \\

\midrule
Ours
& 0.82 $\pm$ 0.04 & 0.96 $\pm$ 0.02 \\
Ours (AR)
& 0.45 $\pm$ 0.04 & 0.70 $\pm$ 0.03 \\
\bottomrule
\end{tabular}
}
\vspace{-0.2cm}
\label{tab:CLIPscore}
\end{table}

